Kernel Distributionally Robust Optimization

We propose kernel distributionally robust optimization (Kernel DRO) using insights from the robust optimization theory and functional analysis. Our method uses reproducing kernel Hilbert spaces (RKHS) to construct a wide range of convex ambiguity sets, which can be generalized to sets based on integral probability metrics and finite-order moment bounds. This perspective unifies multiple existing robust and stochastic optimization methods. We prove a theorem that generalizes the classical duality in the mathematical problem of moments. Enabled by this theorem, we reformulate the maximization with respect to measures in DRO into the dual program that searches for RKHS functions. Using universal RKHSs, the theorem applies to a broad class of loss functions, lifting common limitations such as polynomial losses and knowledge of the Lipschitz constant. We then establish a connection between DRO and stochastic optimization with expectation constraints. Finally, we propose practical algorithms based on both batch convex solvers and stochastic functional gradient, which apply to general optimization and machine learning tasks.

==> draft/additional.tex <==
\subsection{Prove that the constraint is convex}
\begin{proof}
    Let $P_1, P_2\in \mathcal C$, and let  $P = t P_1+(1-t)P_2$, where $t\in[0,1]$. It suffices to show $P\in\mathcal C$ for any choices of $P_1, P_2, t$. Let $\mu_P = \int\phi(x)dP(x)$, we have
    \begin{multline*}
     \|\mu_P - \hat\mu\|_\rkhs= \|t\mu_{P_1} - t\hat\mu +(1-t)\mu_{P_2} - (1-t)\hat\mu\|_\rkhs\\
     \leq \|t\mu_{P_1} - t\hat\mu \|_\rkhs+\|(1-t)\mu_{P_2} - (1-t)\hat\mu\|_\rkhs\\
     \leq t\epsilon + (1-t)\epsilon = \epsilon.
     \end{multline*}
    Hence, $P\in\mathcal C$.
\end{proof}

\subsection{Lemma~\ref{thm:wc_dist_supp} worst-case distribution}
\begin{proof}
    Suppose $\genset$ is a generating class of $\mathcal P$.
    Let us consider the following program
    $$
    \begin{opt1}
        (P'):=\MAXST{P\in \genset,\mu\in \mathcal C}{\int l \ dP}
        {\int{\phi}{\ dP} = \mu},
    \end{opt1}     
    $$
    since $\mathrm{mix}(\genset) = \mathcal P$, the dual of (P') is simply (D). 
    $\genset\cap\mathcal K \neq \emptyset$ implies that the set 
    $$
    \genset_{\mathcal C}:=\{\tau\colon \mu_\tau \in \mathcal C, \tau\in\genset\}
    $$
    has nonempty interior.\jz{or relative interior?} 
    Then (P') is strictly feasible. Let $\tau^*\in\genset$ be the optimal solution of (P'). By strong duality,
    $$
    \pip{l}{\tau^*} = (D'') = (D) = (P),
    $$
    i.e., there exists a measure $\tau^*\in\genset$ that attains the worst-case risk.
\end{proof}

\subsection{$\epsilon$-metric ball case: Worst-case distribution \ref{thm:wc_dist}}
\begin{proof}
    Because $\mathcal C=\{\mu\colon\|\mu - \hat\mu\|_\rkhs\leq \epsilon\}$,
    the set $\genset\cap\mathcal K \neq \emptyset$ at least contains one element $\hat P$.
    Applying \ref{thm:wc_dist_supp}, we obtain the result.
    
    The seond claim is similar.
\end{proof}
From the proof, it is clear that the statement of the reuslt is not true for distributions supported on fewer than $N$ points --- indeed, if we replace $\genset$ with $\mathbb T_{N-1}$, the primal problem might not be feasible and we can not guarantee strong duality in such cases. 
An alternatively proof for a similar result using measure theoretical techniques can be found in \cite{parysDistributionallyRobustControl2015}, Theorem~3.3.

---
Let us consider the well known conditional value-at-risk as a special case of our applciation. \jz{use the simple dual rep. don't use this}
\begin{example}
        (Duchi's form and worst-case conditional value-at-risk)
\begin{multline*}
\min_x\sup_P \mathrm{CVaR}_{\epsilon}(l(x,w)) = \min_x\sup_P\inf_t\{t + \frac1\epsilon\mathbb E\left[l(x,w) - t\right]^+\}\\
= \min_x\inf_t\{t + \sup_P\frac1\epsilon\mathbb E\left[l(x,w) - t\right]^+\} \\
=\inf_t\{t + \min_x\sup_P\frac1\epsilon\mathbb E\left[l(x,w) - t\right]^+\}
\end{multline*}
The function $\mathbb E\left[l(x,w) - t\right]^+$ is convex in $t$. It is convex in $x$ if $l(x,w)$ is convex in $x$. Inspecting the inner min-max problem, we see that this reduces to solving ~\eqref{eq:kdro}. This was extensively studied in operations research such as in \cite{zymlerDistributionallyRobustJoint2013}, Parys, Shapiro risk measure. The authors of [duchi] also discussed using RKHS with this risk measure.
Specifically, they used the approximation
$$
\mathbb E\left[l(x,w) - t\right]^+\approx \sup_{h:\mathcal X\to[0,1]}\mathbb E h(w)(l(x,w) - t)
$$
i.e., using a certain class of functions to approximate the characteristic function $\left[\cdot \right]^+$. They consider the case where $h$ belongs to an RKHS.
\end{example}

%%%%%%%%discuss reduction to krr
Frist, we establish trivial connection between our formulation and kernel-based learning, whose robustness is well-known due to \cite{christmannRobustnessPropertiesConvex, christmannConsistencyRobustnessKernelbased2007}. The proof is by simply constraining the cost funciton in ~\eqref{eq:conic_dual} to be in the RKHS and hence trivial.

\subsection{choquet and rkhs}
If we consider the loss function to be an RKHS function, we obtain the following result that reveals the conneciton between Choquet represetnation and kernel method.
\begin{proof}
        \input{draft/pf/choquet_rkhs.Rmd}
\end{proof}

\section{ball on the ground example}
\begin{figure}[b!]
	\centering
	\includegraphics[width=\columnwidth]{draft/fig/ro_ball.png}
	\caption{Imagine an hyperthetical scenario that we want to simulate a ball on the ground. However, due to reasons such as perception error, we do not known its size accurately, but only an upper bound as in (e). We can simply place the ball to make sure it's above the ground in the \emph{worst-case} scenario. Suppose, to take a data driven approach, we are given samples known to lie inside the ball. We can optionally ensure the mean of samples is above the floor (a), or add to it some margin (b), ensure all samples above the floow (c), or ensure margin around all samples (d). The intuition of (e) is that of the \emph{classical robust optimization} and (a) that of sample average approximation. By properly applying geometric intuition with data, we may improve the performance and strike a balance between performance and robustness. This paper will combine such geometric insights with RKHS theory.}
	\label{fig:ball}
\end{figure}

==> draft/representer.tex <==
Given empirical data $\{\xi_i\}_{i=1}^N$, we define the empirical distribution embedding as $\mu_{\hat P}=\kme{\frac1N}{\xi_i}$.
We give the representation theorem for kernel DRO problem~\eqref{eq:kdro}.
% We now derive a result that states it suffices to consider solutions of the form $\mu_p = \kme{\alpha_i}{x_i}$.
\jz{We will show that contrary to commonly assumed, the bound is not necessarily tight.}

\subsection{Derivation 1}
\begin{equation}
  \begin{aligned}
  &\mnz_x&  &\bigg\{F(x):=\underset{P,\mu}{\sup}  \int l(x,z) \ dP(z) \bigg\}\\
  &\sjt& & \|\mu - \mu_{\hat P}\|_\rkhs\leq \epsilon\\
  % &&& \nu = \mu - \mu_{\hat P}\\
  &&&     \int{\phi(z)}{\ dP(z)} = \mu\\
  &&& P\in \mathcal M, \mu\in \rkhs,
  \end{aligned}
  \label{eq:kdro_signed_meas}
\end{equation}
We note there is a key difference between \eqref{eq:kdro_signed_meas} and \eqref{eq:kdro} is that the worst case measure in \eqref{eq:kdro_signed_meas} may not be a probability measure. 
Nonetheless, we first show the \eqref{eq:kdro_signed_meas} admits the following RKHS representer.

\begin{lemma}
Let $(l^*, \mu_{p^*})$ be the optimal solution pair to \eqref{eq:kdro_signed_meas}. 
Then $l^*$ and  $p^*$ both admit finite-term KME expansion at the given data points., i.e. 
  $$
  l^* = \kme{\beta_i}{\xi_i},  \mu_{p^*} = \kme{\alpha_i}{\xi_i}\\
  $$
  for some $\alpha_i, \beta_i, i=1...N$.
\end{lemma}
  

**Proof** We rewrite the objective as 
$$
\min _ {l\in \mathcal L}   \pip{l}{\mu_{\hat P}}_\rkhs +  \max_{\mu_P} \hip{l'}{\mu_P - \mu_{\hat P}}
$$
By virtue of Cauchy-Schwarz inequality in RKHS, we can analytically solve the inner maximization problem.
$$
\min _ {l\in \mathcal L}   \pip{l}{\mu_{\hat P}}_\rkhs +  \epsilon\hnorm{l}.
$$
The above bound is tight and is attained at $\mu_P = \mu_{\hat P} + \epsilon \frac{l}{\hnorm{l}}$. By the RKHS representer theorem of Schoelkopf et al., we have it that the optimal solution to the above problem can be represented as 
$$
l^* = \kme{\beta_i}{\xi_i}.
$$

Then we naturally obtain
$$
\mu_P = \mu_{\hat P} + \epsilon \frac{l^*}{\hnorm{l^*}}.
$$
Since both of the summands are finitely represented, we have
$$
\mu_{p^*} = \kme{\alpha_i}{\xi_i}
$$
for some $\alpha_i, i=1...N$.


\subsection{Extending to all continuous functions on compact domain}
We now use the fact that some RKHS (e.g. Gaussian) is dense on C[compact] to derive the existence of extremal distributions represented by finitely many kernel expansion.

Given empirical data $\{\xi_i\}_{i=1}^N$, we define the empirical distribution embedding as $\mu_{\hat P}=\kme{\frac1N}{\xi_i}$.
\begin{theorem}
(RKHS representer of extreme distribution)

Let $l$ be a continuous function on a compact domain $\mathcal X$, and $P^*$ be the worst-case distribution of the DRO problem $\ref{eq:dro2}$. For any $\epsilon>0$,  there exists an distribution $P_\epsilon$ such that 
$$
|\pip{l}{P_\epsilon} -\pip{l}{P^*}| \leq\epsilon,
$$
where the RKHS embedding of $P^*$ admits the finite-term representation
$$
\mu_{p_\epsilon} = \kme{\alpha_i}{\xi_i}.
$$
for some $\alpha_i,, i=1...N$.

Further more, if we let $\epsilon\to 0$, we **have**
$$
\mu_{p^*} = \kme{\alpha_i}{\xi_i}.
$$
for some $\alpha_i,, i=1...N$.
\end{theorem}
[**remark**] this theorem tells us that, for solving the DRO problem, it surfices to consider the representation on the empirical expansion. DRO constraint $\| \kme{\alpha^i_t}{\hat x^i} -\kme{\frac1N}{x(u,\xi^i)}\|_\rkhs\leq\epsilon.$ is a robust bound, rather than a sample-based approximation to the $\|P- \hat P\|_{MMD}\leq\epsilon$.

In addition, we don't need to find new expansion points $\xi_i$, which amounts to nonlinear optimization problem such as in [bach herding, chen, welling]

\textbf{proof.}

outline: get $ l'$ such that $|l-l'|_\infty\leq\epsilon_2$, then $p_\epsilon$ is arbitrarily close to true extremal distribution. Then finally, we use the fact that the convergence sequence is Cauchy [need verify].

cf. Apple notes



\subsection{Extremal representation of conv. comb. of Diracs}

If we constrain $\sum\alpha_i = 1$, we imply the extreme distribution is the convex combination of Diracs. This **would be a strong result**!

At least, this is a **robust lower bound**
